Build Your Own Visual-Inertial Drone: A Cost-Effective and Open-Source Autonomous Drone

This paper describes an approach to building a cost-effective and research grade visual-inertial odometry aided vertical taking-off and landing (VTOL) platform. We utilize an off-the-shelf visual-inertial sensor, an onboard computer, and a quadrotor platform that are factory-calibrated and mass-produced, thereby sharing similar hardware and sensor specifications (e.g., mass, dimensions, intrinsic and extrinsic of camera-IMU systems, and signal-to-noise ratio). We then perform a system calibration and identification enabling the use of our visual-inertial odometry, multi-sensor fusion, and model predictive control frameworks with the off-the-shelf products. This implies that we can partially avoid tedious parameter tuning procedures for building a full system. The complete system is extensively evaluated both indoors using a motion capture system and outdoors using a laser tracker while performing hover and step responses, and trajectory following tasks in the presence of external wind disturbances. We achieve root-mean-square (RMS) pose errors between a reference and actual trajectories of 0.036m, while performing hover. We also conduct relatively long distance flight (~180m) experiments on a farm site and achieve 0.82% drift error of the total distance flight. This paper conveys the insights we acquired about the platform and sensor module and returns to the community as open-source code with tutorial documentation.

==> contribs/UseCase.tex <==
% !TEX root = ../RAM_2016_affordable_vi_drone.tex
%========================================================
%		State estimation performance
%========================================================
\subsection{Use-cases}
We present two use-cases for our proposed method of building visual-inertial VTOL platforms. Figure~\ref{fig:use-case} (a) shows a precision agriculture application where the platform carries a visual-inertial sensor and a hyperspectral camera for weed monitoring. (b) depicts a aerial manipulation scenario. These examples illustrate the benefit of the proposed method to perform state estimation and control, and show its reproducibility.
\begin{figure}
\begin{center}
   \subfigure[]{\includegraphics[height=0.3\columnwidth]{./figs/ag_drone.jpeg}}
\subfigure[]{\includegraphics[height=0.3\columnwidth]{./figs/dji_m100.png}}
\end{center}
    \vspace{-5mm}
\caption{Use-cases for (a) precision agriculture (b) and aerial painting.\iks{(b) will be replaced with another image.}}
\label{fig:use-case}
    \vspace{-2mm}
\end{figure}
%\vspace{-3pt}
